Coherent Coupling of a Diamond Tin-Vacancy Center to a Tunable Open Microcavity

Efficient coupling of optically active qubits to optical cavities is a key challenge for solid-state-based quantum optics experiments and future quantum technologies. Here we present a quantum photonic interface based on a single Tin-Vacancy center in a micrometer-thin diamond membrane coupled to a tunable open microcavity. We use the full tunability of the microcavity to selectively address individual Tin-Vacancy centers within the cavity mode volume. Purcell enhancement of the Tin-Vacancy center optical transition is evidenced both by optical excited state lifetime reduction and by optical linewidth broadening. As the emitter selectively reflects the single-photon component of the incident light, the coupled emitter-cavity system exhibits strong quantum nonlinear behavior. On resonance, we observe a transmission dip of 50 % for low incident photon number per Purcell-reduced excited state lifetime, while the dip disappears as the emitter is saturated with higher photon number. Moreover, we demonstrate that the emitter strongly modifies the photon statistics of the transmitted light by observing photon bunching. This work establishes a versatile and tunable platform for advanced quantum optics experiments and proof-of-principle demonstrations towards quantum networking with solid-state qubits.

==> main <==
%apsrev4-2.bst 2019-01-14 (MD) hand-edited version of apsrev4-1.bst
%Control: key (0)
%Control: author (8) initials jnrlst
%Control: editor formatted (1) identically to author
%Control: production of article title (0) allowed
%Control: page (0) single
%Control: year (1) truncated
%Control: production of eprint (0) enabled
\begin{thebibliography}{64}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode
  `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{https://doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
%</preamble>
\bibitem [{\citenamefont {Kimble}(2008)}]{kimble_quantum_2008}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {H.~J.}\ \bibnamefont
  {Kimble}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title}
  {The quantum internet}},\ }\href {https://doi.org/10.1038/nature07127}
  {\bibfield  {journal} {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo
  {volume} {453}},\ \bibinfo {pages} {1023} (\bibinfo {year}
  {2008})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wehner}\ \emph {et~al.}(2018)\citenamefont {Wehner},
  \citenamefont {Elkouss},\ and\ \citenamefont {Hanson}}]{wehner_quantum_2018}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Wehner}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Elkouss}},\
  and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Hanson}},\
  }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title} {Quantum
  internet: {A} vision for the road ahead}},\ }\href
  {https://doi.org/10.1126/science.aam9288} {\bibfield  {journal} {\bibinfo
  {journal} {Science}\ }\textbf {\bibinfo {volume} {362}},\ \bibinfo {pages}
  {eaam9288} (\bibinfo {year} {2018})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Vahala}(2003)}]{vahala_optical_2003}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.~J.}\ \bibnamefont
  {Vahala}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title}
  {Optical microcavities}},\ }\href {https://doi.org/10.1038/nature01939}
  {\bibfield  {journal} {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo
  {volume} {424}},\ \bibinfo {pages} {839} (\bibinfo {year}
  {2003})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Reiserer}\ and\ \citenamefont
  {Rempe}(2015)}]{reiserer_cavity-based_2015}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Reiserer}}\ and\ \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Rempe}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title}
  {Cavity-based quantum networks with single atoms and optical photons}},\
  }\href {https://doi.org/10.1103/RevModPhys.87.1379} {\bibfield  {journal}
  {\bibinfo  {journal} {Rev. Mod. Phys.}\ }\textbf {\bibinfo {volume} {87}},\
  \bibinfo {pages} {1379} (\bibinfo {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Janitz}\ \emph {et~al.}(2020)\citenamefont {Janitz},
  \citenamefont {Bhaskar},\ and\ \citenamefont
  {Childress}}]{janitz_cavity_2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Janitz}}, \bibinfo {author} {\bibfnamefont {M.~K.}\ \bibnamefont
  {Bhaskar}},\ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {Childress}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo
  {title} {Cavity quantum electrodynamics with color centers in diamond}},\
  }\href {https://doi.org/10.1364/OPTICA.398628} {\bibfield  {journal}
  {\bibinfo  {journal} {Optica}\ }\textbf {\bibinfo {volume} {7}},\ \bibinfo
  {pages} {1232} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ruf}\ \emph {et~al.}(2021{\natexlab{a}})\citenamefont
  {Ruf}, \citenamefont {Wan}, \citenamefont {Choi}, \citenamefont {Englund},\
  and\ \citenamefont {Hanson}}]{ruf_quantum_2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Ruf}}, \bibinfo {author} {\bibfnamefont {N.~H.}\ \bibnamefont {Wan}},
  \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Choi}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Englund}},\ and\ \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Hanson}},\ }\bibfield  {title}
  {{\selectlanguage {english}\bibinfo {title} {Quantum networks based on color
  centers in diamond}},\ }\href {https://doi.org/10.1063/5.0056534} {\bibfield
  {journal} {\bibinfo  {journal} {J. Appl. Phys.}\ }\textbf {\bibinfo {volume}
  {130}},\ \bibinfo {pages} {070901} (\bibinfo {year}
  {2021}{\natexlab{a}})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Merkel}\ \emph {et~al.}(2020)\citenamefont {Merkel},
  \citenamefont {Ulanowski},\ and\ \citenamefont
  {Reiserer}}]{merkel_coherent_2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Merkel}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Ulanowski}},\
  and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Reiserer}},\
  }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title} {Coherent and
  {Purcell}-{Enhanced} {Emission} from {Erbium} {Dopants} in a {Cryogenic}
  {High}-{Q} {Resonator}}},\ }\href
  {https://doi.org/10.1103/PhysRevX.10.041025} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. X}\ }\textbf {\bibinfo {volume} {10}},\ \bibinfo
  {pages} {041025} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Casabone}\ \emph {et~al.}(2021)\citenamefont
  {Casabone}, \citenamefont {Deshmukh}, \citenamefont {Liu}, \citenamefont
  {Serrano}, \citenamefont {Ferrier}, \citenamefont {H\"ummer}, \citenamefont
  {Goldner}, \citenamefont {Hunger},\ and\ \citenamefont
  {De~Riedmatten}}]{casabone_dynamic_2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Casabone}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Deshmukh}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Liu}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Serrano}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Ferrier}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {H\"ummer}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Goldner}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Hunger}},\ and\ \bibinfo {author} {\bibfnamefont
  {H.}~\bibnamefont {De~Riedmatten}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Dynamic control of {Purcell} enhanced emission of
  erbium ions in nanoparticles}},\ }\href
  {https://doi.org/10.1038/s41467-021-23632-9} {\bibfield  {journal} {\bibinfo
  {journal} {Nat. Commun.}\ }\textbf {\bibinfo {volume} {12}},\ \bibinfo
  {pages} {3570} (\bibinfo {year} {2021})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Muller}\ \emph {et~al.}(2009)\citenamefont {Muller},
  \citenamefont {Flagg}, \citenamefont {Metcalfe}, \citenamefont {Lawall},\
  and\ \citenamefont {Solomon}}]{muller_coupling_2009}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Muller}}, \bibinfo {author} {\bibfnamefont {E.~B.}\ \bibnamefont {Flagg}},
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Metcalfe}}, \bibinfo
  {author} {\bibfnamefont {J.}~\bibnamefont {Lawall}},\ and\ \bibinfo {author}
  {\bibfnamefont {G.~S.}\ \bibnamefont {Solomon}},\ }\bibfield  {title}
  {{\selectlanguage {english}\bibinfo {title} {Coupling an epitaxial quantum
  dot to a fiber-based external-mirror microcavity}},\ }\href
  {https://doi.org/10.1063/1.3245311} {\bibfield  {journal} {\bibinfo
  {journal} {Appl. Phys. Lett.}\ }\textbf {\bibinfo {volume} {95}},\ \bibinfo
  {pages} {173101} (\bibinfo {year} {2009})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Herzog}\ \emph {et~al.}(2018)\citenamefont {Herzog},
  \citenamefont {Sartison}, \citenamefont {Kolatschek}, \citenamefont {Hepp},
  \citenamefont {Bommer}, \citenamefont {Pauly}, \citenamefont {M\"ucklich},
  \citenamefont {Becher}, \citenamefont {Jetter}, \citenamefont {Portalupi},\
  and\ \citenamefont {Michler}}]{herzog_pure_2018}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Herzog}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Sartison}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Kolatschek}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Hepp}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Bommer}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Pauly}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {M\"ucklich}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Becher}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Jetter}}, \bibinfo {author} {\bibfnamefont {S.~L.}\
  \bibnamefont {Portalupi}},\ and\ \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Michler}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Pure single-photon emission from {In}({Ga}){As}
  {QDs} in a tunable fiber-based external mirror microcavity}},\ }\href
  {https://doi.org/10.1088/2058-9565/aac64d} {\bibfield  {journal} {\bibinfo
  {journal} {Quantum Sci. Technol.}\ }\textbf {\bibinfo {volume} {3}},\
  \bibinfo {pages} {034009} (\bibinfo {year} {2018})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Najer}\ \emph {et~al.}(2019)\citenamefont {Najer},
  \citenamefont {S\"ollner}, \citenamefont {Sekatski}, \citenamefont {Dolique},
  \citenamefont {L\"obl}, \citenamefont {Riedel}, \citenamefont {Schott},
  \citenamefont {Starosielec}, \citenamefont {Valentin}, \citenamefont {Wieck},
  \citenamefont {Sangouard}, \citenamefont {Ludwig},\ and\ \citenamefont
  {Warburton}}]{najer_gated_2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Najer}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {S\"ollner}},
  \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Sekatski}}, \bibinfo
  {author} {\bibfnamefont {V.}~\bibnamefont {Dolique}}, \bibinfo {author}
  {\bibfnamefont {M.~C.}\ \bibnamefont {L\"obl}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Riedel}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Schott}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Starosielec}}, \bibinfo {author} {\bibfnamefont {S.~R.}\
  \bibnamefont {Valentin}}, \bibinfo {author} {\bibfnamefont {A.~D.}\
  \bibnamefont {Wieck}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Sangouard}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Ludwig}},\
  and\ \bibinfo {author} {\bibfnamefont {R.~J.}\ \bibnamefont {Warburton}},\
  }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title} {A gated
  quantum dot strongly coupled to an optical microcavity}},\ }\href
  {https://doi.org/10.1038/s41586-019-1709-y} {\bibfield  {journal} {\bibinfo
  {journal} {Nature}\ }\textbf {\bibinfo {volume} {575}},\ \bibinfo {pages}
  {622} (\bibinfo {year} {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Tomm}\ \emph {et~al.}(2021)\citenamefont {Tomm},
  \citenamefont {Javadi}, \citenamefont {Antoniadis}, \citenamefont {Najer},
  \citenamefont {L\"obl}, \citenamefont {Korsch}, \citenamefont {Schott},
  \citenamefont {Valentin}, \citenamefont {Wieck}, \citenamefont {Ludwig},\
  and\ \citenamefont {Warburton}}]{tomm_bright_2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Tomm}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Javadi}},
  \bibinfo {author} {\bibfnamefont {N.~O.}\ \bibnamefont {Antoniadis}},
  \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Najer}}, \bibinfo
  {author} {\bibfnamefont {M.~C.}\ \bibnamefont {L\"obl}}, \bibinfo {author}
  {\bibfnamefont {A.~R.}\ \bibnamefont {Korsch}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Schott}}, \bibinfo {author} {\bibfnamefont
  {S.~R.}\ \bibnamefont {Valentin}}, \bibinfo {author} {\bibfnamefont {A.~D.}\
  \bibnamefont {Wieck}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Ludwig}},\ and\ \bibinfo {author} {\bibfnamefont {R.~J.}\ \bibnamefont
  {Warburton}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo
  {title} {A bright and fast source of coherent single photons}},\ }\href
  {https://doi.org/10.1038/s41565-020-00831-x} {\bibfield  {journal} {\bibinfo
  {journal} {Nat. Nanotechnol.}\ }\textbf {\bibinfo {volume} {16}},\ \bibinfo
  {pages} {399} (\bibinfo {year} {2021})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {H\"au\ss{}ler}\ \emph {et~al.}(2021)\citenamefont
  {H\"au\ss{}ler}, \citenamefont {Bayer}, \citenamefont {Waltrich},
  \citenamefont {Mendelson}, \citenamefont {Li}, \citenamefont {Hunger},
  \citenamefont {Aharonovich},\ and\ \citenamefont
  {Kubanek}}]{hausler_tunable_2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {H\"au\ss{}ler}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Bayer}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Waltrich}},
  \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Mendelson}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Li}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Hunger}}, \bibinfo {author} {\bibfnamefont
  {I.}~\bibnamefont {Aharonovich}},\ and\ \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Kubanek}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Tunable {Fiber}‐{Cavity} {Enhanced} {Photon}
  {Emission} from {Defect} {Centers} in {hBN}}},\ }\href
  {https://doi.org/10.1002/adom.202002218} {\bibfield  {journal} {\bibinfo
  {journal} {Adv. Opt. Mater.}\ }\textbf {\bibinfo {volume} {9}},\ \bibinfo
  {pages} {2002218} (\bibinfo {year} {2021})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Vadia}\ \emph {et~al.}(2021)\citenamefont {Vadia},
  \citenamefont {Scherzer}, \citenamefont {Thierschmann}, \citenamefont
  {Sch\"afermeier}, \citenamefont {Dal~Savio}, \citenamefont {Taniguchi},
  \citenamefont {Watanabe}, \citenamefont {Hunger}, \citenamefont
  {Karra\"{\i}},\ and\ \citenamefont {H\"ogele}}]{vadia_open-cavity_2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Vadia}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Scherzer}},
  \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Thierschmann}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Sch\"afermeier}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Dal~Savio}}, \bibinfo {author}
  {\bibfnamefont {T.}~\bibnamefont {Taniguchi}}, \bibinfo {author}
  {\bibfnamefont {K.}~\bibnamefont {Watanabe}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Hunger}}, \bibinfo {author} {\bibfnamefont
  {K.}~\bibnamefont {Karra\"{\i}}},\ and\ \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {H\"ogele}},\ }\bibfield  {title} {\bibinfo {title}
  {Open-cavity in closed-cycle cryostat as a quantum optics platform},\ }\href
  {https://doi.org/10.1103/PRXQuantum.2.040318} {\bibfield  {journal} {\bibinfo
   {journal} {PRX Quantum}\ }\textbf {\bibinfo {volume} {2}},\ \bibinfo {pages}
  {040318} (\bibinfo {year} {2021})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wang}\ \emph {et~al.}(2017)\citenamefont {Wang},
  \citenamefont {Kelkar}, \citenamefont {Martin-Cano}, \citenamefont {Utikal},
  \citenamefont {G\"otzinger},\ and\ \citenamefont
  {Sandoghdar}}]{wang_coherent_2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Wang}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Kelkar}},
  \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Martin-Cano}}, \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Utikal}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {G\"otzinger}},\ and\ \bibinfo {author}
  {\bibfnamefont {V.}~\bibnamefont {Sandoghdar}},\ }\bibfield  {title}
  {\bibinfo {title} {Coherent coupling of a single molecule to a scanning
  fabry-perot microcavity},\ }\href {https://doi.org/10.1103/PhysRevX.7.021014}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. X}\ }\textbf {\bibinfo
  {volume} {7}},\ \bibinfo {pages} {021014} (\bibinfo {year}
  {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hunger}\ \emph {et~al.}(2010)\citenamefont {Hunger},
  \citenamefont {Steinmetz}, \citenamefont {Colombe}, \citenamefont {Deutsch},
  \citenamefont {H\"ansch},\ and\ \citenamefont {Reichel}}]{hunger_fiber_2010}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Hunger}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Steinmetz}},
  \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Colombe}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Deutsch}}, \bibinfo {author}
  {\bibfnamefont {T.~W.}\ \bibnamefont {H\"ansch}},\ and\ \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Reichel}},\ }\bibfield  {title}
  {{\selectlanguage {english}\bibinfo {title} {A fiber {Fabry}–{Perot} cavity
  with high finesse}},\ }\href {https://doi.org/10.1088/1367-2630/12/6/065038}
  {\bibfield  {journal} {\bibinfo  {journal} {New J. Phys.}\ }\textbf {\bibinfo
  {volume} {12}},\ \bibinfo {pages} {065038} (\bibinfo {year}
  {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Albrecht}\ \emph {et~al.}(2013)\citenamefont
  {Albrecht}, \citenamefont {Bommer}, \citenamefont {Deutsch}, \citenamefont
  {Reichel},\ and\ \citenamefont {Becher}}]{albrecht_coupling_2013}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Albrecht}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Bommer}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Deutsch}}, \bibinfo
  {author} {\bibfnamefont {J.}~\bibnamefont {Reichel}},\ and\ \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Becher}},\ }\bibfield  {title} {\bibinfo
  {title} {Coupling of a single nitrogen-vacancy center in diamond to a
  fiber-based microcavity},\ }\href
  {https://doi.org/10.1103/PhysRevLett.110.243602} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {110}},\
  \bibinfo {pages} {243602} (\bibinfo {year} {2013})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Johnson}\ \emph {et~al.}(2015)\citenamefont
  {Johnson}, \citenamefont {Dolan}, \citenamefont {Grange}, \citenamefont
  {Trichet}, \citenamefont {Hornecker}, \citenamefont {Chen}, \citenamefont
  {Weng}, \citenamefont {Hughes}, \citenamefont {Watt}, \citenamefont
  {Auff\`{e}ves},\ and\ \citenamefont {Smith}}]{johnson_tunable_2015}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Johnson}}, \bibinfo {author} {\bibfnamefont {P.~R.}\ \bibnamefont {Dolan}},
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Grange}}, \bibinfo
  {author} {\bibfnamefont {A.~A.~P.}\ \bibnamefont {Trichet}}, \bibinfo
  {author} {\bibfnamefont {G.}~\bibnamefont {Hornecker}}, \bibinfo {author}
  {\bibfnamefont {Y.~C.}\ \bibnamefont {Chen}}, \bibinfo {author}
  {\bibfnamefont {L.}~\bibnamefont {Weng}}, \bibinfo {author} {\bibfnamefont
  {G.~M.}\ \bibnamefont {Hughes}}, \bibinfo {author} {\bibfnamefont {A.~A.~R.}\
  \bibnamefont {Watt}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Auff\`{e}ves}},\ and\ \bibinfo {author} {\bibfnamefont {J.~M.}\ \bibnamefont
  {Smith}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title}
  {Tunable cavity coupling of the zero phonon line of a nitrogen-vacancy defect
  in diamond}},\ }\href {https://doi.org/10.1088/1367-2630/17/12/122003}
  {\bibfield  {journal} {\bibinfo  {journal} {New J. Phys.}\ }\textbf {\bibinfo
  {volume} {17}},\ \bibinfo {pages} {122003} (\bibinfo {year}
  {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kaupp}\ \emph {et~al.}(2016)\citenamefont {Kaupp},
  \citenamefont {H\"ummer}, \citenamefont {Mader}, \citenamefont {Schlederer},
  \citenamefont {Benedikter}, \citenamefont {Haeusser}, \citenamefont {Chang},
  \citenamefont {Fedder}, \citenamefont {H\"ansch},\ and\ \citenamefont
  {Hunger}}]{kaupp_purcell-enhanced_2016}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Kaupp}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {H\"ummer}},
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Mader}}, \bibinfo
  {author} {\bibfnamefont {B.}~\bibnamefont {Schlederer}}, \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Benedikter}}, \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Haeusser}}, \bibinfo {author}
  {\bibfnamefont {H.-C.}\ \bibnamefont {Chang}}, \bibinfo {author}
  {\bibfnamefont {H.}~\bibnamefont {Fedder}}, \bibinfo {author} {\bibfnamefont
  {T.~W.}\ \bibnamefont {H\"ansch}},\ and\ \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Hunger}},\ }\bibfield  {title} {\bibinfo {title}
  {Purcell-enhanced single-photon emission from nitrogen-vacancy centers
  coupled to a tunable microcavity},\ }\href
  {https://doi.org/10.1103/PhysRevApplied.6.054010} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Appl.}\ }\textbf {\bibinfo {volume} {6}},\
  \bibinfo {pages} {054010} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Benedikter}\ \emph {et~al.}(2017)\citenamefont
  {Benedikter}, \citenamefont {Kaupp}, \citenamefont {H\"ummer}, \citenamefont
  {Liang}, \citenamefont {Bommer}, \citenamefont {Becher}, \citenamefont
  {Krueger}, \citenamefont {Smith}, \citenamefont {H\"ansch},\ and\
  \citenamefont {Hunger}}]{benedikter_cavity-enhanced_2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Benedikter}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Kaupp}},
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {H\"ummer}}, \bibinfo
  {author} {\bibfnamefont {Y.}~\bibnamefont {Liang}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Bommer}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Becher}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Krueger}}, \bibinfo {author} {\bibfnamefont {J.~M.}\
  \bibnamefont {Smith}}, \bibinfo {author} {\bibfnamefont {T.~W.}\ \bibnamefont
  {H\"ansch}},\ and\ \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Hunger}},\ }\bibfield  {title} {\bibinfo {title} {Cavity-enhanced
  single-photon source based on the silicon-vacancy center in diamond},\ }\href
  {https://doi.org/10.1103/PhysRevApplied.7.024031} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Appl.}\ }\textbf {\bibinfo {volume} {7}},\
  \bibinfo {pages} {024031} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Riedel}\ \emph {et~al.}(2017)\citenamefont {Riedel},
  \citenamefont {S\"ollner}, \citenamefont {Shields}, \citenamefont
  {Starosielec}, \citenamefont {Appel}, \citenamefont {Neu}, \citenamefont
  {Maletinsky},\ and\ \citenamefont {Warburton}}]{riedel_deterministic_2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Riedel}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {S\"ollner}},
  \bibinfo {author} {\bibfnamefont {B.~J.}\ \bibnamefont {Shields}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Starosielec}}, \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Appel}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Neu}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Maletinsky}},\ and\ \bibinfo {author} {\bibfnamefont {R.~J.}\ \bibnamefont
  {Warburton}},\ }\bibfield  {title} {\bibinfo {title} {Deterministic
  enhancement of coherent photon generation from a nitrogen-vacancy center in
  ultrapure diamond},\ }\href {https://doi.org/10.1103/PhysRevX.7.031040}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. X}\ }\textbf {\bibinfo
  {volume} {7}},\ \bibinfo {pages} {031040} (\bibinfo {year}
  {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Salz}\ \emph {et~al.}(2020)\citenamefont {Salz},
  \citenamefont {Herrmann}, \citenamefont {Nadarajah}, \citenamefont {Stahl},
  \citenamefont {Hettrich}, \citenamefont {Stacey}, \citenamefont {Prawer},
  \citenamefont {Hunger},\ and\ \citenamefont
  {Schmidt-Kaler}}]{salz_cryogenic_2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Salz}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Herrmann}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Nadarajah}}, \bibinfo
  {author} {\bibfnamefont {A.}~\bibnamefont {Stahl}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Hettrich}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Stacey}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Prawer}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Hunger}},\ and\ \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Schmidt-Kaler}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Cryogenic platform for coupling color centers in
  diamond membranes to a fiber-based microcavity}},\ }\href
  {https://doi.org/10.1007/s00340-020-07478-5} {\bibfield  {journal} {\bibinfo
  {journal} {Appl. Phys. B}\ }\textbf {\bibinfo {volume} {126}},\ \bibinfo
  {pages} {131} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {H\o{}y~Jensen}\ \emph {et~al.}(2020)\citenamefont
  {H\o{}y~Jensen}, \citenamefont {Janitz}, \citenamefont {Fontana},
  \citenamefont {He}, \citenamefont {Gobron}, \citenamefont {Radko},
  \citenamefont {Bhaskar}, \citenamefont {Evans}, \citenamefont
  {Rodr\'{\i}guez~Rosenblueth}, \citenamefont {Childress}, \citenamefont
  {Huck},\ and\ \citenamefont
  {Lund~Andersen}}]{hoy_jensen_cavity-enhanced_2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {H\o{}y~Jensen}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Janitz}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Fontana}},
  \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {He}}, \bibinfo {author}
  {\bibfnamefont {O.}~\bibnamefont {Gobron}}, \bibinfo {author} {\bibfnamefont
  {I.~P.}\ \bibnamefont {Radko}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Bhaskar}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Evans}}, \bibinfo {author} {\bibfnamefont {C.~D.}\
  \bibnamefont {Rodr\'{\i}guez~Rosenblueth}}, \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Childress}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Huck}},\ and\ \bibinfo {author} {\bibfnamefont
  {U.}~\bibnamefont {Lund~Andersen}},\ }\bibfield  {title} {\bibinfo {title}
  {Cavity-enhanced photon emission from a single germanium-vacancy center in a
  diamond membrane},\ }\href {https://doi.org/10.1103/PhysRevApplied.13.064016}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Appl.}\ }\textbf
  {\bibinfo {volume} {13}},\ \bibinfo {pages} {064016} (\bibinfo {year}
  {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ruf}\ \emph {et~al.}(2021{\natexlab{b}})\citenamefont
  {Ruf}, \citenamefont {Weaver}, \citenamefont {van Dam},\ and\ \citenamefont
  {Hanson}}]{ruf_resonant_2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Ruf}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Weaver}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {van Dam}},\ and\ \bibinfo
  {author} {\bibfnamefont {R.}~\bibnamefont {Hanson}},\ }\bibfield  {title}
  {\bibinfo {title} {Resonant excitation and purcell enhancement of coherent
  nitrogen-vacancy centers coupled to a fabry-perot microcavity},\ }\href
  {https://doi.org/10.1103/PhysRevApplied.15.024049} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Appl.}\ }\textbf {\bibinfo {volume} {15}},\
  \bibinfo {pages} {024049} (\bibinfo {year} {2021}{\natexlab{b}})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Feuchtmayr}\ \emph {et~al.}(2023)\citenamefont
  {Feuchtmayr}, \citenamefont {Berghaus}, \citenamefont {Sachero},
  \citenamefont {Bayer}, \citenamefont {Lettner}, \citenamefont {Waltrich},
  \citenamefont {Maier}, \citenamefont {Agafonov},\ and\ \citenamefont
  {Kubanek}}]{feuchtmayr_enhanced_2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Feuchtmayr}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Berghaus}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Sachero}},
  \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Bayer}}, \bibinfo
  {author} {\bibfnamefont {N.}~\bibnamefont {Lettner}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Waltrich}}, \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Maier}}, \bibinfo {author} {\bibfnamefont
  {V.}~\bibnamefont {Agafonov}},\ and\ \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Kubanek}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Enhanced spectral density of a single germanium
  vacancy center in a nanodiamond by cavity integration}},\ }\href
  {https://doi.org/10.1063/5.0156787} {\bibfield  {journal} {\bibinfo
  {journal} {Appl. Phys. Lett.}\ }\textbf {\bibinfo {volume} {123}},\ \bibinfo
  {pages} {024001} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bayer}\ \emph {et~al.}(2023)\citenamefont {Bayer},
  \citenamefont {Berghaus}, \citenamefont {Sachero}, \citenamefont
  {Filipovski}, \citenamefont {Antoniuk}, \citenamefont {Lettner},
  \citenamefont {Waltrich}, \citenamefont {Klotz}, \citenamefont {Maier},
  \citenamefont {Agafonov},\ and\ \citenamefont
  {Kubanek}}]{bayer_optical_2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Bayer}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Berghaus}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Sachero}}, \bibinfo
  {author} {\bibfnamefont {A.~B.}\ \bibnamefont {Filipovski}}, \bibinfo
  {author} {\bibfnamefont {L.}~\bibnamefont {Antoniuk}}, \bibinfo {author}
  {\bibfnamefont {N.}~\bibnamefont {Lettner}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Waltrich}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Klotz}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Maier}}, \bibinfo {author} {\bibfnamefont
  {V.}~\bibnamefont {Agafonov}},\ and\ \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Kubanek}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Optical driving, spin initialization and readout
  of single {SiV}- centers in a {Fabry}-{Perot} resonator}},\ }\href
  {https://doi.org/10.1038/s42005-023-01422-7} {\bibfield  {journal} {\bibinfo
  {journal} {Commun. Phys.}\ }\textbf {\bibinfo {volume} {6}},\ \bibinfo
  {pages} {300} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bernien}\ \emph {et~al.}(2013)\citenamefont
  {Bernien}, \citenamefont {Hensen}, \citenamefont {Pfaff}, \citenamefont
  {Koolstra}, \citenamefont {Blok}, \citenamefont {Robledo}, \citenamefont
  {Taminiau}, \citenamefont {Markham}, \citenamefont {Twitchen}, \citenamefont
  {Childress},\ and\ \citenamefont {Hanson}}]{bernien_heralded_2013}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Bernien}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Hensen}},
  \bibinfo {author} {\bibfnamefont {W.}~\bibnamefont {Pfaff}}, \bibinfo
  {author} {\bibfnamefont {G.}~\bibnamefont {Koolstra}}, \bibinfo {author}
  {\bibfnamefont {M.~S.}\ \bibnamefont {Blok}}, \bibinfo {author}
  {\bibfnamefont {L.}~\bibnamefont {Robledo}}, \bibinfo {author} {\bibfnamefont
  {T.~H.}\ \bibnamefont {Taminiau}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Markham}}, \bibinfo {author} {\bibfnamefont {D.~J.}\
  \bibnamefont {Twitchen}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {Childress}},\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Hanson}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title}
  {Heralded entanglement between solid-state qubits separated by three
  metres}},\ }\href {https://doi.org/10.1038/nature12016} {\bibfield  {journal}
  {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo {volume} {497}},\ \bibinfo
  {pages} {86} (\bibinfo {year} {2013})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Humphreys}\ \emph {et~al.}(2018)\citenamefont
  {Humphreys}, \citenamefont {Kalb}, \citenamefont {Morits}, \citenamefont
  {Schouten}, \citenamefont {Vermeulen}, \citenamefont {Twitchen},
  \citenamefont {Markham},\ and\ \citenamefont
  {Hanson}}]{humphreys_deterministic_2018}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.~C.}\ \bibnamefont
  {Humphreys}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Kalb}},
  \bibinfo {author} {\bibfnamefont {J.~P.~J.}\ \bibnamefont {Morits}}, \bibinfo
  {author} {\bibfnamefont {R.~N.}\ \bibnamefont {Schouten}}, \bibinfo {author}
  {\bibfnamefont {R.~F.~L.}\ \bibnamefont {Vermeulen}}, \bibinfo {author}
  {\bibfnamefont {D.~J.}\ \bibnamefont {Twitchen}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Markham}},\ and\ \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Hanson}},\ }\bibfield  {title}
  {{\selectlanguage {english}\bibinfo {title} {Deterministic delivery of remote
  entanglement on a quantum network}},\ }\href
  {https://doi.org/10.1038/s41586-018-0200-5} {\bibfield  {journal} {\bibinfo
  {journal} {Nature}\ }\textbf {\bibinfo {volume} {558}},\ \bibinfo {pages}
  {268} (\bibinfo {year} {2018})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bhaskar}\ \emph {et~al.}(2020)\citenamefont
  {Bhaskar}, \citenamefont {Riedinger}, \citenamefont {Machielse},
  \citenamefont {Levonian}, \citenamefont {Nguyen}, \citenamefont {Knall},
  \citenamefont {Park}, \citenamefont {Englund}, \citenamefont {Lon\v{c}ar},
  \citenamefont {Sukachev},\ and\ \citenamefont
  {Lukin}}]{bhaskar_experimental_2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.~K.}\ \bibnamefont
  {Bhaskar}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Riedinger}},
  \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Machielse}}, \bibinfo
  {author} {\bibfnamefont {D.~S.}\ \bibnamefont {Levonian}}, \bibinfo {author}
  {\bibfnamefont {C.~T.}\ \bibnamefont {Nguyen}}, \bibinfo {author}
  {\bibfnamefont {E.~N.}\ \bibnamefont {Knall}}, \bibinfo {author}
  {\bibfnamefont {H.}~\bibnamefont {Park}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Englund}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Lon\v{c}ar}}, \bibinfo {author} {\bibfnamefont {D.~D.}\
  \bibnamefont {Sukachev}},\ and\ \bibinfo {author} {\bibfnamefont {M.~D.}\
  \bibnamefont {Lukin}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Experimental demonstration of memory-enhanced
  quantum communication}},\ }\href {https://doi.org/10.1038/s41586-020-2103-5}
  {\bibfield  {journal} {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo
  {volume} {580}},\ \bibinfo {pages} {60} (\bibinfo {year} {2020})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Abobeih}\ \emph {et~al.}(2018)\citenamefont
  {Abobeih}, \citenamefont {Cramer}, \citenamefont {Bakker}, \citenamefont
  {Kalb}, \citenamefont {Markham}, \citenamefont {Twitchen},\ and\
  \citenamefont {Taminiau}}]{abobeih_one-second_2018}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.~H.}\ \bibnamefont
  {Abobeih}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Cramer}},
  \bibinfo {author} {\bibfnamefont {M.~A.}\ \bibnamefont {Bakker}}, \bibinfo
  {author} {\bibfnamefont {N.}~\bibnamefont {Kalb}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Markham}}, \bibinfo {author} {\bibfnamefont
  {D.~J.}\ \bibnamefont {Twitchen}},\ and\ \bibinfo {author} {\bibfnamefont
  {T.~H.}\ \bibnamefont {Taminiau}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {One-second coherence for a single electron spin
  coupled to a multi-qubit nuclear-spin environment}},\ }\href
  {https://doi.org/10.1038/s41467-018-04916-z} {\bibfield  {journal} {\bibinfo
  {journal} {Nat. Commun.}\ }\textbf {\bibinfo {volume} {9}},\ \bibinfo {pages}
  {2552} (\bibinfo {year} {2018})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Van Der~Sar}\ \emph {et~al.}(2012)\citenamefont {Van
  Der~Sar}, \citenamefont {Wang}, \citenamefont {Blok}, \citenamefont
  {Bernien}, \citenamefont {Taminiau}, \citenamefont {Toyli}, \citenamefont
  {Lidar}, \citenamefont {Awschalom}, \citenamefont {Hanson},\ and\
  \citenamefont {Dobrovitski}}]{van_der_sar_decoherence-protected_2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Van
  Der~Sar}}, \bibinfo {author} {\bibfnamefont {Z.~H.}\ \bibnamefont {Wang}},
  \bibinfo {author} {\bibfnamefont {M.~S.}\ \bibnamefont {Blok}}, \bibinfo
  {author} {\bibfnamefont {H.}~\bibnamefont {Bernien}}, \bibinfo {author}
  {\bibfnamefont {T.~H.}\ \bibnamefont {Taminiau}}, \bibinfo {author}
  {\bibfnamefont {D.~M.}\ \bibnamefont {Toyli}}, \bibinfo {author}
  {\bibfnamefont {D.~A.}\ \bibnamefont {Lidar}}, \bibinfo {author}
  {\bibfnamefont {D.~D.}\ \bibnamefont {Awschalom}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Hanson}},\ and\ \bibinfo {author}
  {\bibfnamefont {V.~V.}\ \bibnamefont {Dobrovitski}},\ }\bibfield  {title}
  {{\selectlanguage {english}\bibinfo {title} {Decoherence-protected quantum
  gates for a hybrid solid-state spin register}},\ }\href
  {https://doi.org/10.1038/nature10900} {\bibfield  {journal} {\bibinfo
  {journal} {Nature}\ }\textbf {\bibinfo {volume} {484}},\ \bibinfo {pages}
  {82} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Stas}\ \emph {et~al.}(2022)\citenamefont {Stas},
  \citenamefont {Huan}, \citenamefont {Machielse}, \citenamefont {Knall},
  \citenamefont {Suleymanzade}, \citenamefont {Pingault}, \citenamefont
  {Sutula}, \citenamefont {Ding}, \citenamefont {Knaut}, \citenamefont
  {Assumpcao}, \citenamefont {Wei}, \citenamefont {Bhaskar}, \citenamefont
  {Riedinger}, \citenamefont {Sukachev}, \citenamefont {Park}, \citenamefont
  {Lon\v{c}ar}, \citenamefont {Levonian},\ and\ \citenamefont
  {Lukin}}]{stas_robust_2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.-J.}\ \bibnamefont
  {Stas}}, \bibinfo {author} {\bibfnamefont {Y.~Q.}\ \bibnamefont {Huan}},
  \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Machielse}}, \bibinfo
  {author} {\bibfnamefont {E.~N.}\ \bibnamefont {Knall}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Suleymanzade}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Pingault}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Sutula}}, \bibinfo {author} {\bibfnamefont
  {S.~W.}\ \bibnamefont {Ding}}, \bibinfo {author} {\bibfnamefont {C.~M.}\
  \bibnamefont {Knaut}}, \bibinfo {author} {\bibfnamefont {D.~R.}\ \bibnamefont
  {Assumpcao}}, \bibinfo {author} {\bibfnamefont {Y.-C.}\ \bibnamefont {Wei}},
  \bibinfo {author} {\bibfnamefont {M.~K.}\ \bibnamefont {Bhaskar}}, \bibinfo
  {author} {\bibfnamefont {R.}~\bibnamefont {Riedinger}}, \bibinfo {author}
  {\bibfnamefont {D.~D.}\ \bibnamefont {Sukachev}}, \bibinfo {author}
  {\bibfnamefont {H.}~\bibnamefont {Park}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Lon\v{c}ar}}, \bibinfo {author} {\bibfnamefont {D.~S.}\
  \bibnamefont {Levonian}},\ and\ \bibinfo {author} {\bibfnamefont {M.~D.}\
  \bibnamefont {Lukin}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Robust multi-qubit quantum network node with
  integrated error detection}},\ }\href
  {https://doi.org/10.1126/science.add9771} {\bibfield  {journal} {\bibinfo
  {journal} {Science}\ }\textbf {\bibinfo {volume} {378}},\ \bibinfo {pages}
  {557} (\bibinfo {year} {2022})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bradley}\ \emph {et~al.}(2019)\citenamefont
  {Bradley}, \citenamefont {Randall}, \citenamefont {Abobeih}, \citenamefont
  {Berrevoets}, \citenamefont {Degen}, \citenamefont {Bakker}, \citenamefont
  {Markham}, \citenamefont {Twitchen},\ and\ \citenamefont
  {Taminiau}}]{bradley_ten-qubit_2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.~E.}\ \bibnamefont
  {Bradley}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Randall}},
  \bibinfo {author} {\bibfnamefont {M.~H.}\ \bibnamefont {Abobeih}}, \bibinfo
  {author} {\bibfnamefont {R.~C.}\ \bibnamefont {Berrevoets}}, \bibinfo
  {author} {\bibfnamefont {M.~J.}\ \bibnamefont {Degen}}, \bibinfo {author}
  {\bibfnamefont {M.~A.}\ \bibnamefont {Bakker}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Markham}}, \bibinfo {author} {\bibfnamefont
  {D.~J.}\ \bibnamefont {Twitchen}},\ and\ \bibinfo {author} {\bibfnamefont
  {T.~H.}\ \bibnamefont {Taminiau}},\ }\bibfield  {title} {\bibinfo {title} {A
  ten-qubit solid-state spin register with quantum memory up to one minute},\
  }\href {https://doi.org/10.1103/PhysRevX.9.031045} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. X}\ }\textbf {\bibinfo {volume} {9}},\
  \bibinfo {pages} {031045} (\bibinfo {year} {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kalb}\ \emph {et~al.}(2017)\citenamefont {Kalb},
  \citenamefont {Reiserer}, \citenamefont {Humphreys}, \citenamefont
  {Bakermans}, \citenamefont {Kamerling}, \citenamefont {Nickerson},
  \citenamefont {Benjamin}, \citenamefont {Twitchen}, \citenamefont {Markham},\
  and\ \citenamefont {Hanson}}]{kalb_entanglement_2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Kalb}}, \bibinfo {author} {\bibfnamefont {A.~A.}\ \bibnamefont {Reiserer}},
  \bibinfo {author} {\bibfnamefont {P.~C.}\ \bibnamefont {Humphreys}}, \bibinfo
  {author} {\bibfnamefont {J.~J.~W.}\ \bibnamefont {Bakermans}}, \bibinfo
  {author} {\bibfnamefont {S.~J.}\ \bibnamefont {Kamerling}}, \bibinfo {author}
  {\bibfnamefont {N.~H.}\ \bibnamefont {Nickerson}}, \bibinfo {author}
  {\bibfnamefont {S.~C.}\ \bibnamefont {Benjamin}}, \bibinfo {author}
  {\bibfnamefont {D.~J.}\ \bibnamefont {Twitchen}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Markham}},\ and\ \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Hanson}},\ }\bibfield  {title}
  {{\selectlanguage {english}\bibinfo {title} {Entanglement distillation
  between solid-state quantum network nodes}},\ }\href
  {https://doi.org/10.1126/science.aan0070} {\bibfield  {journal} {\bibinfo
  {journal} {Science}\ }\textbf {\bibinfo {volume} {356}},\ \bibinfo {pages}
  {928} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hermans}\ \emph {et~al.}(2022)\citenamefont
  {Hermans}, \citenamefont {Pompili}, \citenamefont {Beukers}, \citenamefont
  {Baier}, \citenamefont {Borregaard},\ and\ \citenamefont
  {Hanson}}]{hermans_qubit_2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~L.~N.}\
  \bibnamefont {Hermans}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Pompili}}, \bibinfo {author} {\bibfnamefont {H.~K.~C.}\ \bibnamefont
  {Beukers}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Baier}},
  \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Borregaard}},\ and\
  \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Hanson}},\ }\bibfield
  {title} {{\selectlanguage {english}\bibinfo {title} {Qubit teleportation
  between non-neighbouring nodes in a quantum network}},\ }\href
  {https://doi.org/10.1038/s41586-022-04697-y} {\bibfield  {journal} {\bibinfo
  {journal} {Nature}\ }\textbf {\bibinfo {volume} {605}},\ \bibinfo {pages}
  {663} (\bibinfo {year} {2022})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Knaut}\ \emph {et~al.}(2024)\citenamefont {Knaut},
  \citenamefont {Suleymanzade}, \citenamefont {Wei}, \citenamefont {Assumpcao},
  \citenamefont {Stas}, \citenamefont {Huan}, \citenamefont {Machielse},
  \citenamefont {Knall}, \citenamefont {Sutula}, \citenamefont {Baranes},
  \citenamefont {Sinclair}, \citenamefont {De-Eknamkul}, \citenamefont
  {Levonian}, \citenamefont {Bhaskar}, \citenamefont {Park}, \citenamefont
  {Lončar},\ and\ \citenamefont {Lukin}}]{knaut_entanglement_2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.~M.}\ \bibnamefont
  {Knaut}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Suleymanzade}},
  \bibinfo {author} {\bibfnamefont {Y.-C.}\ \bibnamefont {Wei}}, \bibinfo
  {author} {\bibfnamefont {D.~R.}\ \bibnamefont {Assumpcao}}, \bibinfo {author}
  {\bibfnamefont {P.-J.}\ \bibnamefont {Stas}}, \bibinfo {author}
  {\bibfnamefont {Y.~Q.}\ \bibnamefont {Huan}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Machielse}}, \bibinfo {author}
  {\bibfnamefont {E.~N.}\ \bibnamefont {Knall}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Sutula}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Baranes}}, \bibinfo {author} {\bibfnamefont
  {N.}~\bibnamefont {Sinclair}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {De-Eknamkul}}, \bibinfo {author} {\bibfnamefont {D.~S.}\
  \bibnamefont {Levonian}}, \bibinfo {author} {\bibfnamefont {M.~K.}\
  \bibnamefont {Bhaskar}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Park}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Lončar}},\ and\
  \bibinfo {author} {\bibfnamefont {M.~D.}\ \bibnamefont {Lukin}},\ }\bibfield
  {title} {\bibinfo {title} {Entanglement of nanophotonic quantum memory nodes
  in a telecom network},\ }\href {https://doi.org/10.1038/s41586-024-07252-z}
  {\bibfield  {journal} {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo
  {volume} {629}},\ \bibinfo {pages} {573–578} (\bibinfo {year}
  {2024})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Janitz}\ \emph {et~al.}(2015)\citenamefont {Janitz},
  \citenamefont {Ruf}, \citenamefont {Dimock}, \citenamefont {Bourassa},
  \citenamefont {Sankey},\ and\ \citenamefont
  {Childress}}]{janitz_fabry-perot_2015}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Janitz}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Ruf}},
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Dimock}}, \bibinfo
  {author} {\bibfnamefont {A.}~\bibnamefont {Bourassa}}, \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Sankey}},\ and\ \bibinfo {author}
  {\bibfnamefont {L.}~\bibnamefont {Childress}},\ }\bibfield  {title}
  {{\selectlanguage {english}\bibinfo {title} {Fabry-{Perot} microcavity for
  diamond-based photonics}},\ }\href
  {https://doi.org/10.1103/PhysRevA.92.043844} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo {volume} {92}},\ \bibinfo
  {pages} {043844} (\bibinfo {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Trusheim}\ \emph {et~al.}(2020)\citenamefont
  {Trusheim}, \citenamefont {Pingault}, \citenamefont {Wan}, \citenamefont
  {G\"undo\ifmmode~\breve{g}\else \u{g}\fi{}an}, \citenamefont {De~Santis},
  \citenamefont {Debroux}, \citenamefont {Gangloff}, \citenamefont {Purser},
  \citenamefont {Chen}, \citenamefont {Walsh}, \citenamefont {Rose},
  \citenamefont {Becker}, \citenamefont {Lienhard}, \citenamefont {Bersin},
  \citenamefont {Paradeisanos}, \citenamefont {Wang}, \citenamefont {Lyzwa},
  \citenamefont {Montblanch}, \citenamefont {Malladi}, \citenamefont {Bakhru},
  \citenamefont {Ferrari}, \citenamefont {Walmsley}, \citenamefont
  {Atat\"ure},\ and\ \citenamefont
  {Englund}}]{trusheim_transform-limited_2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.~E.}\ \bibnamefont
  {Trusheim}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Pingault}},
  \bibinfo {author} {\bibfnamefont {N.~H.}\ \bibnamefont {Wan}}, \bibinfo
  {author} {\bibfnamefont {M.}~\bibnamefont {G\"undo\ifmmode~\breve{g}\else
  \u{g}\fi{}an}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {De~Santis}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Debroux}},
  \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Gangloff}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Purser}}, \bibinfo {author}
  {\bibfnamefont {K.~C.}\ \bibnamefont {Chen}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Walsh}}, \bibinfo {author} {\bibfnamefont
  {J.~J.}\ \bibnamefont {Rose}}, \bibinfo {author} {\bibfnamefont {J.~N.}\
  \bibnamefont {Becker}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Lienhard}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Bersin}},
  \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Paradeisanos}}, \bibinfo
  {author} {\bibfnamefont {G.}~\bibnamefont {Wang}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Lyzwa}}, \bibinfo {author} {\bibfnamefont
  {A.~R.-P.}\ \bibnamefont {Montblanch}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Malladi}}, \bibinfo {author} {\bibfnamefont
  {H.}~\bibnamefont {Bakhru}}, \bibinfo {author} {\bibfnamefont {A.~C.}\
  \bibnamefont {Ferrari}}, \bibinfo {author} {\bibfnamefont {I.~A.}\
  \bibnamefont {Walmsley}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Atat\"ure}},\ and\ \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Englund}},\ }\bibfield  {title} {\bibinfo {title} {Transform-limited photons
  from a coherent tin-vacancy spin in diamond},\ }\href
  {https://doi.org/10.1103/PhysRevLett.124.023602} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {124}},\
  \bibinfo {pages} {023602} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rugar}\ \emph {et~al.}(2020)\citenamefont {Rugar},
  \citenamefont {Dory}, \citenamefont {Aghaeimeibodi}, \citenamefont {Lu},
  \citenamefont {Sun}, \citenamefont {Mishra}, \citenamefont {Shen},
  \citenamefont {Melosh},\ and\ \citenamefont {Vu\ifmmode \check{c}\else
  \v{c}\fi{}kovi\ifmmode~\acute{c}\else
  \'{c}\fi{}}}]{rugar_narrow-linewidth_2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~E.}\ \bibnamefont
  {Rugar}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Dory}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Aghaeimeibodi}}, \bibinfo
  {author} {\bibfnamefont {H.}~\bibnamefont {Lu}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Sun}}, \bibinfo {author} {\bibfnamefont
  {S.~D.}\ \bibnamefont {Mishra}}, \bibinfo {author} {\bibfnamefont {Z.-X.}\
  \bibnamefont {Shen}}, \bibinfo {author} {\bibfnamefont {N.~A.}\ \bibnamefont
  {Melosh}},\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Vu\ifmmode \check{c}\else \v{c}\fi{}kovi\ifmmode~\acute{c}\else
  \'{c}\fi{}}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo
  {title} {Narrow-{Linewidth} {Tin}-{Vacancy} {Centers} in a {Diamond}
  {Waveguide}}},\ }\href {https://doi.org/10.1021/acsphotonics.0c00833}
  {\bibfield  {journal} {\bibinfo  {journal} {ACS Photonics}\ }\textbf
  {\bibinfo {volume} {7}},\ \bibinfo {pages} {2356} (\bibinfo {year}
  {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Arjona~Mart\'{\i}nez}\ \emph
  {et~al.}(2022)\citenamefont {Arjona~Mart\'{\i}nez}, \citenamefont {Parker},
  \citenamefont {Chen}, \citenamefont {Purser}, \citenamefont {Li},
  \citenamefont {Michaels}, \citenamefont {Stramma}, \citenamefont {Debroux},
  \citenamefont {Harris}, \citenamefont {Hayhurst~Appel}, \citenamefont
  {Nichols}, \citenamefont {Trusheim}, \citenamefont {Gangloff}, \citenamefont
  {Englund},\ and\ \citenamefont {Atat\"ure}}]{arjona_martinez_photonic_2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Arjona~Mart\'{\i}nez}}, \bibinfo {author} {\bibfnamefont {R.~A.}\
  \bibnamefont {Parker}}, \bibinfo {author} {\bibfnamefont {K.~C.}\
  \bibnamefont {Chen}}, \bibinfo {author} {\bibfnamefont {C.~M.}\ \bibnamefont
  {Purser}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Li}}, \bibinfo
  {author} {\bibfnamefont {C.~P.}\ \bibnamefont {Michaels}}, \bibinfo {author}
  {\bibfnamefont {A.~M.}\ \bibnamefont {Stramma}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Debroux}}, \bibinfo {author} {\bibfnamefont
  {I.~B.}\ \bibnamefont {Harris}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Hayhurst~Appel}}, \bibinfo {author} {\bibfnamefont
  {E.~C.}\ \bibnamefont {Nichols}}, \bibinfo {author} {\bibfnamefont {M.~E.}\
  \bibnamefont {Trusheim}}, \bibinfo {author} {\bibfnamefont {D.~A.}\
  \bibnamefont {Gangloff}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Englund}},\ and\ \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Atat\"ure}},\ }\bibfield  {title} {\bibinfo {title} {Photonic
  indistinguishability of the tin-vacancy center in nanostructured diamond},\
  }\href {https://doi.org/10.1103/PhysRevLett.129.173603} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {129}},\
  \bibinfo {pages} {173603} (\bibinfo {year} {2022})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rosenthal}\ \emph {et~al.}(2023)\citenamefont
  {Rosenthal}, \citenamefont {Anderson}, \citenamefont {Kleidermacher},
  \citenamefont {Stein}, \citenamefont {Lee}, \citenamefont {Grzesik},
  \citenamefont {Scuri}, \citenamefont {Rugar}, \citenamefont {Riedel},
  \citenamefont {Aghaeimeibodi}, \citenamefont {Ahn}, \citenamefont
  {Van~Gasse},\ and\ \citenamefont {Vu\ifmmode \check{c}\else
  \v{c}\fi{}kovi\ifmmode~\acute{c}\else
  \'{c}\fi{}}}]{rosenthal_microwave_2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.~I.}\ \bibnamefont
  {Rosenthal}}, \bibinfo {author} {\bibfnamefont {C.~P.}\ \bibnamefont
  {Anderson}}, \bibinfo {author} {\bibfnamefont {H.~C.}\ \bibnamefont
  {Kleidermacher}}, \bibinfo {author} {\bibfnamefont {A.~J.}\ \bibnamefont
  {Stein}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Lee}}, \bibinfo
  {author} {\bibfnamefont {J.}~\bibnamefont {Grzesik}}, \bibinfo {author}
  {\bibfnamefont {G.}~\bibnamefont {Scuri}}, \bibinfo {author} {\bibfnamefont
  {A.~E.}\ \bibnamefont {Rugar}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Riedel}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Aghaeimeibodi}}, \bibinfo {author} {\bibfnamefont {G.~H.}\
  \bibnamefont {Ahn}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Van~Gasse}},\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Vu\ifmmode \check{c}\else \v{c}\fi{}kovi\ifmmode~\acute{c}\else
  \'{c}\fi{}}},\ }\bibfield  {title} {\bibinfo {title} {Microwave spin control
  of a tin-vacancy qubit in diamond},\ }\href
  {https://doi.org/10.1103/PhysRevX.13.031022} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. X}\ }\textbf {\bibinfo {volume} {13}},\ \bibinfo
  {pages} {031022} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Guo}\ \emph {et~al.}(2023)\citenamefont {Guo},
  \citenamefont {Stramma}, \citenamefont {Li}, \citenamefont {Roth},
  \citenamefont {Huang}, \citenamefont {Jin}, \citenamefont {Parker},
  \citenamefont {Arjona~Mart\'{\i}nez}, \citenamefont {Shofer}, \citenamefont
  {Michaels}, \citenamefont {Purser}, \citenamefont {Appel}, \citenamefont
  {Alexeev}, \citenamefont {Liu}, \citenamefont {Ferrari}, \citenamefont
  {Awschalom}, \citenamefont {Delegan}, \citenamefont {Pingault}, \citenamefont
  {Galli}, \citenamefont {Heremans}, \citenamefont {Atat\"ure},\ and\
  \citenamefont {High}}]{guo_microwave-based_2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {X.}~\bibnamefont
  {Guo}}, \bibinfo {author} {\bibfnamefont {A.~M.}\ \bibnamefont {Stramma}},
  \bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont {Li}}, \bibinfo {author}
  {\bibfnamefont {W.~G.}\ \bibnamefont {Roth}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Huang}}, \bibinfo {author} {\bibfnamefont
  {Y.}~\bibnamefont {Jin}}, \bibinfo {author} {\bibfnamefont {R.~A.}\
  \bibnamefont {Parker}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Arjona~Mart\'{\i}nez}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Shofer}}, \bibinfo {author} {\bibfnamefont {C.~P.}\ \bibnamefont
  {Michaels}}, \bibinfo {author} {\bibfnamefont {C.~P.}\ \bibnamefont
  {Purser}}, \bibinfo {author} {\bibfnamefont {M.~H.}\ \bibnamefont {Appel}},
  \bibinfo {author} {\bibfnamefont {E.~M.}\ \bibnamefont {Alexeev}}, \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Liu}}, \bibinfo {author}
  {\bibfnamefont {A.~C.}\ \bibnamefont {Ferrari}}, \bibinfo {author}
  {\bibfnamefont {D.~D.}\ \bibnamefont {Awschalom}}, \bibinfo {author}
  {\bibfnamefont {N.}~\bibnamefont {Delegan}}, \bibinfo {author} {\bibfnamefont
  {B.}~\bibnamefont {Pingault}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Galli}}, \bibinfo {author} {\bibfnamefont {F.~J.}\
  \bibnamefont {Heremans}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Atat\"ure}},\ and\ \bibinfo {author} {\bibfnamefont {A.~A.}\ \bibnamefont
  {High}},\ }\bibfield  {title} {\bibinfo {title} {Microwave-based quantum
  control and coherence protection of tin-vacancy spin qubits in a strain-tuned
  diamond-membrane heterostructure},\ }\href
  {https://doi.org/10.1103/PhysRevX.13.041037} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. X}\ }\textbf {\bibinfo {volume} {13}},\ \bibinfo
  {pages} {041037} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ruf}\ \emph {et~al.}(2019)\citenamefont {Ruf},
  \citenamefont {IJspeert}, \citenamefont {van Dam}, \citenamefont {de~Jong},
  \citenamefont {van~den Berg}, \citenamefont {Evers},\ and\ \citenamefont
  {Hanson}}]{ruf_optically_2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Ruf}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {IJspeert}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {van Dam}}, \bibinfo
  {author} {\bibfnamefont {N.}~\bibnamefont {de~Jong}}, \bibinfo {author}
  {\bibfnamefont {H.}~\bibnamefont {van~den Berg}}, \bibinfo {author}
  {\bibfnamefont {G.}~\bibnamefont {Evers}},\ and\ \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Hanson}},\ }\bibfield  {title}
  {{\selectlanguage {english}\bibinfo {title} {Optically {Coherent}
  {Nitrogen}-{Vacancy} {Centers} in {Micrometer}-{Thin} {Etched} {Diamond}
  {Membranes}}},\ }\href {https://doi.org/10.1021/acs.nanolett.9b01316}
  {\bibfield  {journal} {\bibinfo  {journal} {Nano Lett.}\ }\textbf {\bibinfo
  {volume} {19}},\ \bibinfo {pages} {3987} (\bibinfo {year}
  {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Appel}\ \emph {et~al.}(2016)\citenamefont {Appel},
  \citenamefont {Neu}, \citenamefont {Ganzhorn}, \citenamefont {Barfuss},
  \citenamefont {Batzer}, \citenamefont {Gratz}, \citenamefont {Tsch\"ope},\
  and\ \citenamefont {Maletinsky}}]{appel_fabrication_2016}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Appel}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Neu}}, \bibinfo
  {author} {\bibfnamefont {M.}~\bibnamefont {Ganzhorn}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Barfuss}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Batzer}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Gratz}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Tsch\"ope}},\ and\ \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Maletinsky}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Fabrication of all diamond scanning probes for
  nanoscale magnetometry}},\ }\href {https://doi.org/10.1063/1.4952953}
  {\bibfield  {journal} {\bibinfo  {journal} {Rev. Sci. Instrum.}\ }\textbf
  {\bibinfo {volume} {87}},\ \bibinfo {pages} {063703} (\bibinfo {year}
  {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {van Dam}\ \emph {et~al.}(2018)\citenamefont {van
  Dam}, \citenamefont {Ruf},\ and\ \citenamefont
  {Hanson}}]{van_dam_optimal_2018}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~B.}\ \bibnamefont
  {van Dam}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Ruf}},\ and\
  \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Hanson}},\ }\bibfield
  {title} {{\selectlanguage {english}\bibinfo {title} {Optimal design of
  diamond-air microcavities for quantum networks using an analytical
  approach}},\ }\href {https://doi.org/10.1088/1367-2630/aaec29} {\bibfield
  {journal} {\bibinfo  {journal} {New J. Phys.}\ }\textbf {\bibinfo {volume}
  {20}},\ \bibinfo {pages} {115004} (\bibinfo {year} {2018})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Herrmann}\ \emph {et~al.}(2024)\citenamefont
  {Herrmann}, \citenamefont {Fischer}, \citenamefont {Scheijen}, \citenamefont
  {Wolfs}, \citenamefont {Brevoord}, \citenamefont {Sauerzapf}, \citenamefont
  {Wienhoven}, \citenamefont {Feije}, \citenamefont {Eschen}, \citenamefont
  {Ruf}, \citenamefont {Weaver},\ and\ \citenamefont
  {Hanson}}]{herrmann_low-temperature_2024}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont
  {Herrmann}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Fischer}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Scheijen}}, \bibinfo
  {author} {\bibfnamefont {C.~F.~J.}\ \bibnamefont {Wolfs}}, \bibinfo {author}
  {\bibfnamefont {J.~M.}\ \bibnamefont {Brevoord}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Sauerzapf}}, \bibinfo {author}
  {\bibfnamefont {L.~G.~C.}\ \bibnamefont {Wienhoven}}, \bibinfo {author}
  {\bibfnamefont {L.~J.}\ \bibnamefont {Feije}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Eschen}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Ruf}}, \bibinfo {author} {\bibfnamefont {M.~J.}\
  \bibnamefont {Weaver}},\ and\ \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Hanson}},\ }\href {https://arxiv.org/abs/2409.01857}
  {\bibinfo {title} {A low-temperature tunable microcavity featuring high
  passive stability and microwave integration}} (\bibinfo {year} {2024}),\
  \Eprint {https://arxiv.org/abs/2409.01857} {arXiv:2409.01857 [quant-ph]}
  \BibitemShut {NoStop}%
\bibitem [{\citenamefont {G\"orlitz}\ \emph {et~al.}(2020)\citenamefont
  {G\"orlitz}, \citenamefont {Herrmann}, \citenamefont {Thiering},
  \citenamefont {Fuchs}, \citenamefont {Gandil}, \citenamefont {Iwasaki},
  \citenamefont {Taniguchi}, \citenamefont {Kieschnick}, \citenamefont
  {Meijer}, \citenamefont {Hatano}, \citenamefont {Gali},\ and\ \citenamefont
  {Becher}}]{gorlitz_spectroscopic_2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {G\"orlitz}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Herrmann}},
  \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Thiering}}, \bibinfo
  {author} {\bibfnamefont {P.}~\bibnamefont {Fuchs}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Gandil}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Iwasaki}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Taniguchi}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Kieschnick}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Meijer}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Hatano}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Gali}},\ and\ \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Becher}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Spectroscopic investigations of negatively charged
  tin-vacancy centres in diamond}},\ }\href
  {https://doi.org/10.1088/1367-2630/ab6631} {\bibfield  {journal} {\bibinfo
  {journal} {New J. Phys.}\ }\textbf {\bibinfo {volume} {22}},\ \bibinfo
  {pages} {013048} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Iwasaki}\ \emph {et~al.}(2017)\citenamefont
  {Iwasaki}, \citenamefont {Miyamoto}, \citenamefont {Taniguchi}, \citenamefont
  {Siyushev}, \citenamefont {Metsch}, \citenamefont {Jelezko},\ and\
  \citenamefont {Hatano}}]{iwasaki_tin-vacancy_2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Iwasaki}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Miyamoto}},
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Taniguchi}}, \bibinfo
  {author} {\bibfnamefont {P.}~\bibnamefont {Siyushev}}, \bibinfo {author}
  {\bibfnamefont {M.~H.}\ \bibnamefont {Metsch}}, \bibinfo {author}
  {\bibfnamefont {F.}~\bibnamefont {Jelezko}},\ and\ \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Hatano}},\ }\bibfield  {title} {\bibinfo
  {title} {Tin-vacancy quantum emitters in diamond},\ }\href
  {https://doi.org/10.1103/PhysRevLett.119.253601} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {119}},\
  \bibinfo {pages} {253601} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rugar}\ \emph {et~al.}(2021)\citenamefont {Rugar},
  \citenamefont {Aghaeimeibodi}, \citenamefont {Riedel}, \citenamefont {Dory},
  \citenamefont {Lu}, \citenamefont {McQuade}, \citenamefont {Shen},
  \citenamefont {Melosh},\ and\ \citenamefont {Vu\ifmmode \check{c}\else
  \v{c}\fi{}kovi\ifmmode~\acute{c}\else \'{c}\fi{}}}]{rugar_quantum_2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~E.}\ \bibnamefont
  {Rugar}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Aghaeimeibodi}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Riedel}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Dory}},
  \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Lu}}, \bibinfo {author}
  {\bibfnamefont {P.~J.}\ \bibnamefont {McQuade}}, \bibinfo {author}
  {\bibfnamefont {Z.-X.}\ \bibnamefont {Shen}}, \bibinfo {author}
  {\bibfnamefont {N.~A.}\ \bibnamefont {Melosh}},\ and\ \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Vu\ifmmode \check{c}\else
  \v{c}\fi{}kovi\ifmmode~\acute{c}\else \'{c}\fi{}}},\ }\bibfield  {title}
  {\bibinfo {title} {Quantum photonic interface for tin-vacancy centers in
  diamond},\ }\href {https://doi.org/10.1103/PhysRevX.11.031021} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. X}\ }\textbf {\bibinfo {volume}
  {11}},\ \bibinfo {pages} {031021} (\bibinfo {year} {2021})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Borregaard}\ \emph {et~al.}(2019)\citenamefont
  {Borregaard}, \citenamefont {Sørensen},\ and\ \citenamefont
  {Lodahl}}]{borregaard_quantum_2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Borregaard}}, \bibinfo {author} {\bibfnamefont {A.~S.}\ \bibnamefont
  {Sørensen}},\ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Lodahl}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title}
  {Quantum {Networks} with {Deterministic} {Spin}–{Photon} {Interfaces}}},\
  }\href {https://doi.org/10.1002/qute.201800091} {\bibfield  {journal}
  {\bibinfo  {journal} {Adv. Quantum Technol.}\ }\textbf {\bibinfo {volume}
  {2}},\ \bibinfo {pages} {1800091} (\bibinfo {year} {2019})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Jahnke}\ \emph {et~al.}(2015)\citenamefont {Jahnke},
  \citenamefont {Sipahigil}, \citenamefont {Binder}, \citenamefont {Doherty},
  \citenamefont {Metsch}, \citenamefont {Rogers}, \citenamefont {Manson},
  \citenamefont {Lukin},\ and\ \citenamefont
  {Jelezko}}]{jahnke_electronphonon_2015}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.~D.}\ \bibnamefont
  {Jahnke}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Sipahigil}},
  \bibinfo {author} {\bibfnamefont {J.~M.}\ \bibnamefont {Binder}}, \bibinfo
  {author} {\bibfnamefont {M.~W.}\ \bibnamefont {Doherty}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Metsch}}, \bibinfo {author} {\bibfnamefont
  {L.~J.}\ \bibnamefont {Rogers}}, \bibinfo {author} {\bibfnamefont {N.~B.}\
  \bibnamefont {Manson}}, \bibinfo {author} {\bibfnamefont {M.~D.}\
  \bibnamefont {Lukin}},\ and\ \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Jelezko}},\ }\bibfield  {title} {{\selectlanguage
  {english}\bibinfo {title} {Electron–phonon processes of the silicon-vacancy
  centre in diamond}},\ }\href {https://doi.org/10.1088/1367-2630/17/4/043011}
  {\bibfield  {journal} {\bibinfo  {journal} {New J. Phys.}\ }\textbf {\bibinfo
  {volume} {17}},\ \bibinfo {pages} {043011} (\bibinfo {year}
  {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wang}\ \emph {et~al.}(2024)\citenamefont {Wang},
  \citenamefont {Kazak}, \citenamefont {Senkalla}, \citenamefont {Siyushev},
  \citenamefont {Abe}, \citenamefont {Taniguchi}, \citenamefont {Onoda},
  \citenamefont {Kato}, \citenamefont {Makino}, \citenamefont {Hatano},
  \citenamefont {Jelezko},\ and\ \citenamefont
  {Iwasaki}}]{wang_transform-limited_2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Wang}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Kazak}},
  \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Senkalla}}, \bibinfo
  {author} {\bibfnamefont {P.}~\bibnamefont {Siyushev}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Abe}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Taniguchi}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Onoda}}, \bibinfo {author} {\bibfnamefont
  {H.}~\bibnamefont {Kato}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Makino}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Hatano}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Jelezko}},\ and\ \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Iwasaki}},\ }\bibfield  {title}
  {\bibinfo {title} {Transform-limited photon emission from a lead-vacancy
  center in diamond above 10 k},\ }\href
  {https://doi.org/10.1103/PhysRevLett.132.073601} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {132}},\
  \bibinfo {pages} {073601} (\bibinfo {year} {2024})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Thompson}\ \emph {et~al.}(1992)\citenamefont
  {Thompson}, \citenamefont {Rempe},\ and\ \citenamefont
  {Kimble}}]{thompson_observation_1992}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.~J.}\ \bibnamefont
  {Thompson}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Rempe}},\
  and\ \bibinfo {author} {\bibfnamefont {H.~J.}\ \bibnamefont {Kimble}},\
  }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title} {Observation
  of normal-mode splitting for an atom in an optical cavity}},\ }\href
  {https://doi.org/10.1103/PhysRevLett.68.1132} {\bibfield  {journal} {\bibinfo
   {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {68}},\ \bibinfo
  {pages} {1132} (\bibinfo {year} {1992})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sipahigil}\ \emph {et~al.}(2016)\citenamefont
  {Sipahigil}, \citenamefont {Evans}, \citenamefont {Sukachev}, \citenamefont
  {Burek}, \citenamefont {Borregaard}, \citenamefont {Bhaskar}, \citenamefont
  {Nguyen}, \citenamefont {Pacheco}, \citenamefont {Atikian}, \citenamefont
  {Meuwly}, \citenamefont {Camacho}, \citenamefont {Jelezko}, \citenamefont
  {Bielejec}, \citenamefont {Park}, \citenamefont {Lon\v{c}ar},\ and\
  \citenamefont {Lukin}}]{sipahigil_integrated_2016}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Sipahigil}}, \bibinfo {author} {\bibfnamefont {R.~E.}\ \bibnamefont
  {Evans}}, \bibinfo {author} {\bibfnamefont {D.~D.}\ \bibnamefont {Sukachev}},
  \bibinfo {author} {\bibfnamefont {M.~J.}\ \bibnamefont {Burek}}, \bibinfo
  {author} {\bibfnamefont {J.}~\bibnamefont {Borregaard}}, \bibinfo {author}
  {\bibfnamefont {M.~K.}\ \bibnamefont {Bhaskar}}, \bibinfo {author}
  {\bibfnamefont {C.~T.}\ \bibnamefont {Nguyen}}, \bibinfo {author}
  {\bibfnamefont {J.~L.}\ \bibnamefont {Pacheco}}, \bibinfo {author}
  {\bibfnamefont {H.~A.}\ \bibnamefont {Atikian}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Meuwly}}, \bibinfo {author} {\bibfnamefont
  {R.~M.}\ \bibnamefont {Camacho}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Jelezko}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Bielejec}}, \bibinfo {author} {\bibfnamefont
  {H.}~\bibnamefont {Park}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Lon\v{c}ar}},\ and\ \bibinfo {author} {\bibfnamefont {M.~D.}\ \bibnamefont
  {Lukin}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title}
  {An integrated diamond nanophotonics platform for quantum-optical
  networks}},\ }\href {https://doi.org/10.1126/science.aah6875} {\bibfield
  {journal} {\bibinfo  {journal} {Science}\ }\textbf {\bibinfo {volume}
  {354}},\ \bibinfo {pages} {847} (\bibinfo {year} {2016})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Lukin}\ \emph {et~al.}(2020)\citenamefont {Lukin},
  \citenamefont {Guidry},\ and\ \citenamefont {Vu\ifmmode \check{c}\else
  \v{c}\fi{}kovi\ifmmode~\acute{c}\else \'{c}\fi{}}}]{lukin_integrated_2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.~M.}\ \bibnamefont
  {Lukin}}, \bibinfo {author} {\bibfnamefont {M.~A.}\ \bibnamefont {Guidry}},\
  and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Vu\ifmmode
  \check{c}\else \v{c}\fi{}kovi\ifmmode~\acute{c}\else \'{c}\fi{}}},\
  }\bibfield  {title} {\bibinfo {title} {Integrated quantum photonics with
  silicon carbide: Challenges and prospects},\ }\href
  {https://doi.org/10.1103/PRXQuantum.1.020102} {\bibfield  {journal} {\bibinfo
   {journal} {PRX Quantum}\ }\textbf {\bibinfo {volume} {1}},\ \bibinfo {pages}
  {020102} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Heiler}\ \emph {et~al.}(2024)\citenamefont {Heiler},
  \citenamefont {K\"{o}rber}, \citenamefont {Hesselmeier}, \citenamefont
  {Kuna}, \citenamefont {St\"{o}hr}, \citenamefont {Fuchs}, \citenamefont
  {Ghezellou}, \citenamefont {Ul-Hassan}, \citenamefont {Knolle}, \citenamefont
  {Becher}, \citenamefont {Kaiser},\ and\ \citenamefont
  {Wrachtrup}}]{heiler_spectral_2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Heiler}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {K\"{o}rber}},
  \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Hesselmeier}}, \bibinfo
  {author} {\bibfnamefont {P.}~\bibnamefont {Kuna}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {St\"{o}hr}}, \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Fuchs}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Ghezellou}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Ul-Hassan}}, \bibinfo {author} {\bibfnamefont
  {W.}~\bibnamefont {Knolle}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Becher}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Kaiser}},\ and\ \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Wrachtrup}},\ }\bibfield  {title} {\bibinfo {title}
  {Spectral stability of v2 centres in sub-micron 4h-sic membranes},\
  }\bibfield  {journal} {\bibinfo  {journal} {npj Quantum Materials}\ }\textbf
  {\bibinfo {volume} {9}},\ \href {https://doi.org/10.1038/s41535-024-00644-4}
  {10.1038/s41535-024-00644-4} (\bibinfo {year} {2024})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bogdanovi\'c}\ \emph
  {et~al.}(2017{\natexlab{a}})\citenamefont {Bogdanovi\'c}, \citenamefont {van
  Dam}, \citenamefont {Bonato}, \citenamefont {Coenen}, \citenamefont
  {Zwerver}, \citenamefont {Hensen}, \citenamefont {Liddy}, \citenamefont
  {Fink}, \citenamefont {Reiserer}, \citenamefont {Lon\v{c}ar},\ and\
  \citenamefont {Hanson}}]{bogdanovic_design_2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Bogdanovi\'c}}, \bibinfo {author} {\bibfnamefont {S.~B.}\ \bibnamefont {van
  Dam}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Bonato}}, \bibinfo
  {author} {\bibfnamefont {L.~C.}\ \bibnamefont {Coenen}}, \bibinfo {author}
  {\bibfnamefont {A.-M.~J.}\ \bibnamefont {Zwerver}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Hensen}}, \bibinfo {author} {\bibfnamefont
  {M.~S.~Z.}\ \bibnamefont {Liddy}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Fink}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Reiserer}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Lon\v{c}ar}},\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Hanson}},\ }\bibfield  {title} {{\selectlanguage {english}\bibinfo {title}
  {Design and low-temperature characterization of a tunable microcavity for
  diamond-based quantum networks}},\ }\href {https://doi.org/10.1063/1.4982168}
  {\bibfield  {journal} {\bibinfo  {journal} {Appl. Phys. Lett.}\ }\textbf
  {\bibinfo {volume} {110}},\ \bibinfo {pages} {171103} (\bibinfo {year}
  {2017}{\natexlab{a}})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Flågan}\ \emph {et~al.}(2022)\citenamefont
  {Flågan}, \citenamefont {Riedel}, \citenamefont {Javadi}, \citenamefont
  {Jakubczyk}, \citenamefont {Maletinsky},\ and\ \citenamefont
  {Warburton}}]{flagan_diamond-confined_2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Flågan}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Riedel}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Javadi}}, \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Jakubczyk}}, \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Maletinsky}},\ and\ \bibinfo {author}
  {\bibfnamefont {R.~J.}\ \bibnamefont {Warburton}},\ }\bibfield  {title}
  {{\selectlanguage {english}\bibinfo {title} {A diamond-confined open
  microcavity featuring a high quality-factor and a small mode-volume}},\
  }\href {https://doi.org/10.1063/5.0081577} {\bibfield  {journal} {\bibinfo
  {journal} {J. Appl. Phys.}\ }\textbf {\bibinfo {volume} {131}},\ \bibinfo
  {pages} {113102} (\bibinfo {year} {2022})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {K\"orber}\ \emph {et~al.}(2023)\citenamefont
  {K\"orber}, \citenamefont {Pallmann}, \citenamefont {Heupel}, \citenamefont
  {St\"ohr}, \citenamefont {Vasilenko}, \citenamefont {H\"ummer}, \citenamefont
  {Kohler}, \citenamefont {Popov},\ and\ \citenamefont
  {Hunger}}]{korber_scanning_2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {K\"orber}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Pallmann}},
  \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Heupel}}, \bibinfo
  {author} {\bibfnamefont {R.}~\bibnamefont {St\"ohr}}, \bibinfo {author}
  {\bibfnamefont {E.}~\bibnamefont {Vasilenko}}, \bibinfo {author}
  {\bibfnamefont {T.}~\bibnamefont {H\"ummer}}, \bibinfo {author}
  {\bibfnamefont {L.}~\bibnamefont {Kohler}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Popov}},\ and\ \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Hunger}},\ }\bibfield  {title} {\bibinfo {title} {Scanning
  cavity microscopy of a single-crystal diamond membrane},\ }\href
  {https://doi.org/10.1103/PhysRevApplied.19.064057} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Appl.}\ }\textbf {\bibinfo {volume} {19}},\
  \bibinfo {pages} {064057} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bogdanovi\'c}\ \emph
  {et~al.}(2017{\natexlab{b}})\citenamefont {Bogdanovi\'c}, \citenamefont
  {Liddy}, \citenamefont {van Dam}, \citenamefont {Coenen}, \citenamefont
  {Fink}, \citenamefont {Lon\v{c}ar},\ and\ \citenamefont
  {Hanson}}]{bogdanovic_robust_2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Bogdanovi\'c}}, \bibinfo {author} {\bibfnamefont {M.~S.~Z.}\ \bibnamefont
  {Liddy}}, \bibinfo {author} {\bibfnamefont {S.~B.}\ \bibnamefont {van Dam}},
  \bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont {Coenen}}, \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Fink}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Lon\v{c}ar}},\ and\ \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Hanson}},\ }\bibfield  {title}
  {{\selectlanguage {english}\bibinfo {title} {Robust nano-fabrication of an
  integrated platform for spin control in a tunable microcavity}},\ }\href
  {https://doi.org/10.1063/1.5001144} {\bibfield  {journal} {\bibinfo
  {journal} {APL Photonics}\ }\textbf {\bibinfo {volume} {2}},\ \bibinfo
  {pages} {126101} (\bibinfo {year} {2017}{\natexlab{b}})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Herrmann}\ \emph {et~al.}(2023)\citenamefont
  {Herrmann}, \citenamefont {Fischer}, \citenamefont {Brevoord}, \citenamefont
  {Sauerzapf}, \citenamefont {Wienhoven}, \citenamefont {Feije}, \citenamefont
  {Pasini}, \citenamefont {Eschen}, \citenamefont {Ruf}, \citenamefont
  {Weaver},\ and\ \citenamefont {Hanson}}]{herrmann_data_2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont
  {Herrmann}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Fischer}},
  \bibinfo {author} {\bibfnamefont {J.~M.}\ \bibnamefont {Brevoord}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Sauerzapf}}, \bibinfo {author}
  {\bibfnamefont {L.~G.~C.}\ \bibnamefont {Wienhoven}}, \bibinfo {author}
  {\bibfnamefont {L.~J.}\ \bibnamefont {Feije}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Pasini}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Eschen}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Ruf}}, \bibinfo {author} {\bibfnamefont {M.~J.}\
  \bibnamefont {Weaver}},\ and\ \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Hanson}},\ }\href
  {https://doi.org/10.4121/421a26ac-4e92-411f-bb0a-5e6af21cf426}
  {{\selectlanguage {english}\bibinfo {title} {Data underlying the publication
  "{Coherent} {Coupling} of a {Diamond} {Tin}-{Vacancy} {Center} to a {Tunable}
  {Open} {Microcavity}"}}} (\bibinfo {year} {2023})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Raa}\ \emph {et~al.}(2023)\citenamefont {Raa},
  \citenamefont {Ervasti}, \citenamefont {Botma}, \citenamefont {Visser},
  \citenamefont {Budhrani}, \citenamefont {van Rantwijk}, \citenamefont
  {Cadot}, \citenamefont {Vermeltfoort}, \citenamefont {Pompili}, \citenamefont
  {Stolk}, \citenamefont {Weaver}, \citenamefont {van~der Enden}, \citenamefont
  {de~Leeuw~Duarte}, \citenamefont {Teng}, \citenamefont {van Zwieten},\ and\
  \citenamefont {Grooteman}}]{raa_qmi_2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {I.~T.}\ \bibnamefont
  {Raa}}, \bibinfo {author} {\bibfnamefont {H.~K.}\ \bibnamefont {Ervasti}},
  \bibinfo {author} {\bibfnamefont {P.~J.}\ \bibnamefont {Botma}}, \bibinfo
  {author} {\bibfnamefont {L.~C.}\ \bibnamefont {Visser}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Budhrani}}, \bibinfo {author}
  {\bibfnamefont {J.~F.}\ \bibnamefont {van Rantwijk}}, \bibinfo {author}
  {\bibfnamefont {S.~P.}\ \bibnamefont {Cadot}}, \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Vermeltfoort}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Pompili}}, \bibinfo {author} {\bibfnamefont
  {A.~J.}\ \bibnamefont {Stolk}}, \bibinfo {author} {\bibfnamefont {M.~J.}\
  \bibnamefont {Weaver}}, \bibinfo {author} {\bibfnamefont {K.~L.}\
  \bibnamefont {van~der Enden}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {de~Leeuw~Duarte}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Teng}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {van Zwieten}},\ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Grooteman}},\ }\href
  {https://doi.org/10.4121/6D39C6DB-2F50-4A49-AD60-5BB08F40CB52} {\bibinfo
  {title} {{QMI} - {Quantum} {Measurement} {Infrastructure}, a {Python} 3
  framework for controlling laboratory equipment}} (\bibinfo {year}
  {2023})\BibitemShut {NoStop}%
\bibitem [{Note1()}]{Note1}%
  \BibitemOpen
  \bibinfo {note} {Available under: \protect \url
  {https://gitlab.com/quantify-os/quantify-core}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Johansson}\ \emph {et~al.}(2012)\citenamefont
  {Johansson}, \citenamefont {Nation},\ and\ \citenamefont
  {Nori}}]{johansson_qutip_2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Johansson}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Nation}},\
  and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Nori}},\ }\bibfield
  {title} {{\selectlanguage {english}\bibinfo {title} {{QuTiP}: {An}
  open-source {Python} framework for the dynamics of open quantum systems}},\
  }\href {https://doi.org/10.1016/j.cpc.2012.02.021} {\bibfield  {journal}
  {\bibinfo  {journal} {Comput. Phys. Commun.}\ }\textbf {\bibinfo {volume}
  {183}},\ \bibinfo {pages} {1760} (\bibinfo {year} {2012})}\BibitemShut
  {NoStop}%
\end{thebibliography}%

